Manifold-based Verbalizer Space Re-embedding for Tuning-free Prompt-based Classification

Prompt-based classification adapts tasks to a cloze question format utilizing the [MASK] token and the filled tokens are then mapped to labels through pre-defined verbalizers. Recent studies have explored the use of verbalizer embeddings to reduce labor in this process. However, all existing studies require a tuning process for either the pre-trained models or additional trainable embeddings. Meanwhile, the distance between high-dimensional verbalizer embeddings should not be measured by Euclidean distance due to the potential for non-linear manifolds in the representation space. In this study, we propose a tuning-free manifold-based space re-embedding method called Locally Linear Embedding with Intra-class Neighborhood Constraint (LLE-INC) for verbalizer embeddings, which preserves local properties within the same class as guidance for classification. Experimental results indicate that even without tuning any parameters, our LLE-INC is on par with automated verbalizers with parameter tuning. And with the parameter updating, our approach further enhances prompt-based tuning by up to 3.2%. Furthermore, experiments with the LLaMA-7B&13B indicate that LLE-INC is an efficient tuning-free classification approach for the hyper-scale language models.

==> Text/3.background.tex <==
% \section{Background}
% No content here

==> Text/8._Limitation___Ethics.tex <==
\section*{Limitations}
Our study re-embedded the prompt verbalizer space by leveraging the local neighborhood feature within the same class and LLE-INC can perform fairly well with tuning \textit{no} parameter. The space reconstruction relies on the neighbor embeddings from the same class and with an extremely limited number of neighbors, such as 2 or 4, it can be challenging for LLE-INC to effectively re-embed the verbalizer space. As the number of neighbors or training instances increases, the performance of LLE-INC improves. Additionally, the dimension of the re-embedded space can be considered as a hyper-parameter, similar to the batch size and learning rate, and the experimental results in Section \ref{hyper} indicate that the performance may exhibit a specific trend with varying dimensions.

\section*{Ethics Statement}
In this study, we present an approach, LLE-INC, for re-embedding the prompt verbalizer space. We conduct our experiments on the publicly available datasets from the GLUE, CBLUE and CLUE benchmarks. All experimental datasets, including those in the biomedical domain have been de-identified by the dataset providers and only used exclusively for research purposes.

==> Text/rebuttal.tex <==
\section{Response to All Reviewers} 
We thank all the reviewers for their thoughtful comments! We are encouraged that they find our approach novel (R4), interesting and efficient (R1), cost-saving (R1, R3), technical and reasonable (R3), inspiring (R4), easy to follow and well-written (R1, R4, R5). We will answer the questions below but incorporate all feedback.

\section{Response to Review 1}
\textbf{Q1: Performance on LLaMA-65B.} \\ 
\noindent A1: We didn't try the LLaMA-65B due to the computational cost and page limit. We tried to conduct the experiments with LLaMA-65B and reported the results in Table 7. It is noticeable that LLaMA-65B with our LLE-INC (-$\blacksquare$) is still superior to that without re-embedding (-$\blacktriangle$).
\begin{table}[hbtp]
\centering
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{lccccccc}
\hline
\hline
&  \textbf{SST-2} & \textbf{MRPC}   & \textbf{QQP} & \textbf{MNLI} &  \textbf{QNLI}  & \textbf{RTE}  \\ \hline

L-13B-$\blacksquare$ \dag  &\textbf{93.8} &82.9&79.2 &70.1 & 76.2       & 79.1        \\

L-13B-$\blacktriangle$ \dag     & 88.8  &   80.6   &  75.6    & 64.9   &  73.9  & 73.0 \\ \hline

L-65B-$\blacksquare$ \dag  &92.8&\textbf{83.0}&\textbf{81.7} &\textbf{73.5} & \textbf{84.3}        & \textbf{83.4}        \\

L-65B-$\blacktriangle$ \dag    & 86.8  &   81.2   & 77.4    & 66.2   &   79.1 & 73.6 \\
 \hline \hline
\end{tabular}
}

\caption{Experimental results for LLaMA-13B and LLaMA-65B. \dag: tuning-free (without the contrastive learning module). $\blacksquare$ denotes the LLE-INC space re-embedding (LLaMA-LLE-INC \dag \ in Table 2). $\blacktriangle$ denotes no re-embedding (LLaMA-w/o re-embed \dag \ in Table 2).}
\label{table:ablation-llama}
\end{table}

\noindent \textbf{Comment 1: It sounds obvious that intra-class information is helpful.} \\
\noindent R1: Although the utilization of intra-class instances is conventionally recognized as beneficial, our LLE-INC innovatively employs intra-class instances \textit{in a tuning-free manner}. LLE-INC re-embeds the representation space for the prompt verbalizer with the constraint of the intra-class neighborhood, so the intra-class information functions as the guidance of tuning-free space re-embedding for a better distance metric in the Euclidean space. Meanwhile, various tuning methods relying on the training sets can refine the model performance, yet with the computational cost of fine-tuning, which is proportional to the scale of the language models. In contrast, LLE-INC can be an efficient solution for large language models to learn from the training sets without parameter updating. \\

\noindent \textbf{Comment 2: The role of ablation study} \\
\noindent R2: The sections of ``Re-embedding Strategy'' and ``Ablation Study'' are both analyses for exploring the effects of specific modules of our approach. In the ``Re-embedding Strategy'' section, we experimented with different re-embedding approaches, including (1) our proposed LLE-INC, (2) original LLE without intra-class information, and (3) no re-embedding to demonstrate the efficacy of our LLE-INC. Meanwhile, in the ``Ablation Study'' section, we experimented with (1) only LLE-INC, (2) only contrastive learning, and (3) a combination of both, to demonstrate only contrastive learning cannot achieve satisfactory performance for the parameter updating. And \textit{LLE-INC is effective for both the tuning-free and parameter-updating scenarios}. \\

\noindent \textbf{Comment 3: Analysis of proposed method} \\
\noindent R3: In this study, we have focused on the \textit{application and performance improvement} with our approach. Therefore, we conducted experiments including (1) tuning-free with LLE-INC, (2) parameter-updating with LLE-INC and contrastive learning, (3) original LLE-based re-embedding without the intra-class information, (4) only kNN without re-embedding, (5) experiments on LLaMA-7B, 13B and 65B (in this page) parameters to extend the usability on large language models. To provide a more comprehensive analysis of our methods, we will incorporate the \textit{theoretical derivation and visualization} as further analysis in the final version of our paper if our paper is accepted.

\section{Response to Review 3}
\textbf{Q1: In Figure 3, why the re-embedded representation of a training instance is put into the LLE-INC model again?} \\
\noindent A1: The arrow from ``the re-embedded $\hat{h}_{\mathtt{[MASK]}}$ of training instances'' to the ``LLE-INC'' for the ``testing instances'' denotes that the LLE-INC for testing instances is built depending on the training instances. We will adjust the figure for easier understanding.\\

\noindent \textbf{Q2: Details of mathematical proof in Step 2.}\\
\noindent A2: We will provide the complete mathematical derivation in the final version of our paper if our paper is accepted.\\

\noindent \textbf{Q3: Mathematical notation, details of verbalizer (and code for the paper)}\\
\noindent A3: Due to the page limit, we placed (1) the notation table for the variables and parameters involved in this study in Table 5, and (2) the implementation of prompt template and verbalizer along with the hyper-parameters in the Appendix file named ``LLE-INC-appendix.pdf'' \textbf{\textit{in the supplementary files}}. We also attached our code in the supplementary files. Please refer to them for more information.

\section{Response to Review 4}
Thank you for your generous and encouraging comments, which not only uplift our spirits but also enhance the quality of our work.

\section{Response to Review 5}
\noindent \textbf{Q: Contribution is limited and the model seems like a variant of contrastive learning.}\\
\noindent A: The main contribution of our research is the development of an innovative method that leverages training datasets through a \textit{tuning-free approach} with (large) language models. Notably, the manifold-based re-embedding constitutes the cornerstone of our method, significantly enhancing the efficacy of distance metrics by reconstructing the embedding space. Contrastive learning functions as \textit{a supplementary component} to infuse task-specific information into the models, thus further enhancing the models with LLE-INC, which means contrastive learning is \textit{not essential} for our approach. Experiments with LLaMA 7B,13B, and 65B which are \textit{free from contrastive learning}, have proved the efficacy of LLE-INC.






